ID-to-3D: Expressive ID-guided 3D Heads via Score Distillation Sampling

We propose ID-to-3D, a method to generate identity- and text-guided 3D human heads with disentangled expressions, starting from even a single casually captured in-the-wild image of a subject. The foundation of our approach is anchored in compositionality, alongside the use of task-specific 2D diffusion models as priors for optimization. First, we extend a foundational model with a lightweight expression-aware and ID-aware architecture, and create 2D priors for geometry and texture generation, via fine-tuning only 0.2% of its available training parameters. Then, we jointly leverage a neural parametric representation for the expressions of each subject and a multi-stage generation of highly detailed geometry and albedo texture. This combination of strong face identity embeddings and our neural representation enables accurate reconstruction of not only facial features but also accessories and hair and can be meshed to provide render-ready assets for gaming and telepresence. Our results achieve an unprecedented level of identity-consistent and high-quality texture and geometry generation, generalizing to a ``world'' of unseen 3D identities, without relying on large 3D captured datasets of human assets.

==> Tables/table.tex <==
\begin{table}
    \centering
    \begin{tabular}{lcc}
        \toprule
        \textbf{ } & \textbf{Shaded} & \textbf{Normals} \\
        \midrule
        Fantasia3D & 252 & 159 \\
        TADA & 215 & 118 \\
        DreamFace & 185 & 140 \\
        HumanNorm & 164 & 98  \\\hline
        Magic123 & 162 & 180 \\
        DreamCraft3D & 205 & 165 \\\hline
        Ours & 153 & 85  \\
      \bottomrule
    \end{tabular}
    \caption{Frechet Inception Distance}
    \label{tab:freq}
\end{table}
